Mixed Diffusion for 3D Indoor Scene Synthesis

Generating realistic 3D scenes is an area of growing interest in computer vision and robotics. However, creating high-quality, diverse synthetic 3D content often requires expert intervention, making it costly and complex. Recently, efforts to automate this process with learning techniques, particularly diffusion models, have shown significant improvements in tasks like furniture rearrangement. However, applying diffusion models to floor-conditioned indoor scene synthesis remains under-explored. This task is especially challenging as it requires arranging objects in continuous space while selecting from discrete object categories, posing unique difficulties for conventional diffusion methods. To bridge this gap, we present MiDiffusion, a novel mixed discrete-continuous diffusion model designed to synthesize plausible 3D indoor scenes given a floor plan and pre-arranged objects. We represent a scene layout by a 2D floor plan and a set of objects, each defined by category, location, size, and orientation. Our approach uniquely applies structured corruption across mixed discrete semantic and continuous geometric domains, resulting in a better-conditioned problem for denoising. Evaluated on the 3D-FRONT dataset, MiDiffusion outperforms state-of-the-art autoregressive and diffusion models in floor-conditioned 3D scene synthesis. Additionally, it effectively handles partial object constraints via a corruption-and-masking strategy without task-specific training, demonstrating advantages in scene completion and furniture arrangement tasks.

==> figure/extreme_layout/extreme_layout.tex <==
\begin{figure}[!ht]
\vspace{-0.2cm}
    \centering
    % bedrooms
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0079_Bedroom-9787.png}
    \end{minipage}%
    \hfill
    \begin{minipage}{0.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0034_Bedroom-11398.png}
    \end{minipage}
    \hfill
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0030_MasterBedroom-81302.png}
    \end{minipage}%
    \hfill
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0010_MasterBedroom-29735.png}
    \end{minipage}%
    \hfill
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0017_LivingDiningRoom-126918.png}
    \end{minipage}%
    % todo
    \\
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0059_LivingDiningRoom-37001.png}
    \end{minipage}%
    \hfill
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0018_LivingRoom-7106.png}
    \end{minipage}%
    \hfill
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0085_LivingDiningRoom-126918.png}
    \end{minipage}%
    \hfill
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0045_LivingDiningRoom-98003.png}
    \end{minipage}%
    \hfill
    \begin{minipage}{.195\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/extreme_layout/0068_DiningRoom-11628.png}
    \end{minipage}%
    % 
    \caption*{Figure: Example results given out-of-distribution floor plans. (to be added to Appendix F)}
    % \vspace{-1cm}
\end{figure}

==> figure/rendered_layouts/rendered_layouts.tex <==
% scene ids: 19, 47, 62. 67

\begin{figure}
    \centering
    % \vspace{-0.1cm}
    \begin{minipage}[t]{0.15\textwidth}
       ATISS\\~\cite{Paschalidou21neurips-ATISS}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/atiss/0019_SecondBedroom-30334.png}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/atiss/0047_MasterBedroom-196.png}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/atiss/0062_MasterBedroom-40255.png}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/atiss/0047_MasterBedroom-196.png}
    \end{minipage}%
    % \vspace{-0.1cm}

    \centering
    \begin{minipage}[t]{0.15\textwidth}
       DiffuScene\\~\cite{Tang24cvpr-DiffuScene}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/diffuscene/0019_SecondBedroom-30334.png}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/diffuscene/0047_MasterBedroom-196.png}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/diffuscene/0062_MasterBedroom-40255.png}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/diffuscene/0047_MasterBedroom-196.png}
    \end{minipage}%
    % \vspace{-0.1cm}
    
    \centering
    \begin{minipage}[t]{0.15\textwidth}
    \algorithm\\
       (Ours)
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/midiffusion/0019_SecondBedroom-30334.png}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/midiffusion/0047_MasterBedroom-196.png}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/midiffusion/0062_MasterBedroom-40255.png}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/midiffusion/0047_MasterBedroom-196.png}
    \end{minipage}%
    % \vspace{-0.1cm}

    \centering
    \begin{minipage}[t]{0.15\textwidth}
    GT
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/gt/0019_SecondBedroom-30334.png}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/gt/0047_MasterBedroom-196.png}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/gt/0062_MasterBedroom-40255.png}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/gt/0067_MasterBedroom-10364.png}
    \end{minipage}%
    \caption{Example bedroom top-down orthographic projection images for quantitative evaluations.}
    \hfill


    \centering
    % \vspace{-0.1cm}
    \begin{minipage}[t]{0.15\textwidth}
       ATISS\\~\cite{Paschalidou21neurips-ATISS}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/atiss/0002_DiningRoom-17147.png}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/atiss/0014_LivingDiningRoom-13177.png}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/atiss/0036_DiningRoom-85692.png}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/atiss/0037_LivingDiningRoom-941.png}
    \end{minipage}%
    % \vspace{-0.1cm}

    \centering
    \begin{minipage}[t]{0.15\textwidth}
       DiffuScene\\~\cite{Tang24cvpr-DiffuScene}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/diffuscene/0002_DiningRoom-17147.png}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/diffuscene/0014_LivingDiningRoom-13177.png}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/diffuscene/0036_DiningRoom-85692.png}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/diffuscene/0037_LivingDiningRoom-941.png}
    \end{minipage}%
    % \vspace{-0.1cm}
    
    \centering
    \begin{minipage}[t]{0.15\textwidth}
    \algorithm\\
       (Ours)
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/midiffusion/0002_DiningRoom-17147.png}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/midiffusion/0014_LivingDiningRoom-13177.png}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/midiffusion/0036_DiningRoom-85692.png}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/midiffusion/0037_LivingDiningRoom-941.png}
    \end{minipage}%
    % \vspace{-0.1cm}

    \centering
    \begin{minipage}[t]{0.15\textwidth}
    GT
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/gt/0002_DiningRoom-17147.png}
    \end{minipage}%
    \begin{minipage}{0.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/gt/0014_LivingDiningRoom-13177.png}
    \end{minipage}
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/gt/0036_DiningRoom-85692.png}
    \end{minipage}%
    \begin{minipage}{.2\textwidth}
        \centering
        \includegraphics[width=0.95\linewidth]{figure/rendered_layouts/gt/0037_LivingDiningRoom-941.png}
    \end{minipage}%
    \caption{Example dining room top-down orthographic projection images for quantitative evaluations.}
    \label{fig:diningroom_rendered_layouts}
    \label{fig:bedroom_rendered_layouts}
    %\vspace{-1.6cm}
\end{figure}

==> tab/scene_completion_additional.tex <==
%!TEX root = ../main.tex

% floor conditioned layout synthesis with existing objects - additional results

\begin{table}[ht]
\vspace{-0.2cm}
\resizebox{\textwidth}{!}{
\begin{tabular}{llcccclcccclcccc}
\hline
\multirow{2}{*}{Method} &  & \multicolumn{4}{c}{Bedroom}  &  & \multicolumn{4}{c}{Dining room} &  & \multicolumn{4}{c}{Living room} \\ \cline{3-6} \cline{8-11} \cline{13-16} 
            &  & FID   &KIDx0.001& CA \%   &KLx0.01&  & FID   &KIDx0.001& CA \%   &\small{KLx0.01}&  & FID   &KIDx0.001& CA \%   &KLx0.01\\ \hline
ATISS       &  & 51.83          & -0.57 & 56.89 +/- 3.86          & \textbf{0.66}          &  & 33.53          & 5.39          & 55.31 +/- 4.54          & 1.60          &  & 31.78          & 5.39          & 59.53 +/- 4.78          & 1.43          \\
DiffuScene  &  & \textbf{42.77} & \textbf{-1.08} & \textbf{52.26 +/- 1.10} & 0.80          &  & 30.58          & 3.67          & 53.67 +/- 4.35          & \textbf{0.84} &  & 32.07          & 4.58          & 59.80 +/- 4.38          & \textbf{0.57} \\
\algorithm(Ours)        &  & 51.87          & -0.34 & 57.44 +/- 4.01    & 0.70      &  & \textbf{28.01} & \textbf{2.03} & \textbf{52.57 +/- 3.10} & 1.72          &  & \textbf{28.74} & \textbf{1.97} & \textbf{57.60 +/- 4.31} & 0.97         \\
 \hline
\end{tabular}
}
\caption{Evaluation results for scene completion given 3 existing objects. \label{tab:scene_completion}} 
% \vspace{-0.4cm}
\end{table}



==> tab/scene_completion_obj.tex <==
%!TEX root = ../main.tex

% scene completion

\begin{table}[ht]
% \vspace{-0.5cm}
\centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{llccclccclccc}
\hline
\multirow{2}{*}{Method} &  & \multicolumn{3}{c}{Bedroom}  &  & \multicolumn{3}{c}{Dining room} &  & \multicolumn{3}{c}{Living room} \\ \cline{3-5} \cline{7-9} \cline{11-13} 
           &  & Obj           & OOB \%        & IoU \%         & & Obj            & OOB \%         & IoU \%         & & Obj            & OOB \%        & IoU \%         \\ \hline
ATISS      &  & 5.50          & 8.89          & 0.84          & & 11.67          & 12.26         & 1.73          &  & 12.91          & 13.03         & 1.29          \\
DiffuScene &  & \textbf{5.29} & 5.13          & \textbf{0.32} & & \textbf{11.12} & 10.04         & \textbf{0.74} & & \textbf{12.29} & 16.13         & \textbf{0.54} \\
\algorithm(Ours)       &  & 5.86          & \textbf{4.05} & 0.74          & & 11.58          & \textbf{4.08} & 1.004          & & 12.81          & \textbf{7.17} & 0.72          \\ \hline
GT         &  & 5.22          & 3.37          & 0.24          & & 11.11          & 0.73          & 0.48          & & 11.67          & 1.55          & 0.27     \\ \hline
\end{tabular}
}
\caption{Bounding box evaluations for scene completion given 3 existing objects. \label{tab:scene_completion_obj}} 
% \vspace{-0.5cm}
\end{table}
